Object Agnostic 3D Lifting in Space and Time

We present a spatio-temporal perspective on category-agnostic 3D lifting of 2D keypoints over a temporal sequence. Our approach differs from existing state-of-the-art methods that are either: (i) object-agnostic, but can only operate on individual frames, or (ii) can model space-time dependencies, but are only designed to work with a single object category. Our approach is grounded in two core principles. First, general information about similar objects can be leveraged to achieve better performance when there is little object-specific training data. Second, a temporally-proximate context window is advantageous for achieving consistency throughout a sequence. These two principles allow us to outperform current state-of-the-art methods on per-frame and per-sequence metrics for a variety of animal categories. Lastly, we release a new synthetic dataset containing 3D skeletons and motion sequences for a variety of animal categories.

==> figures/main_fig.tex <==
\begin{figure*}
  \centering
  
  % \subfloat[3D-LFM]{
  %   \includegraphics[width=0.45\linewidth]{rabbit_3dlfm2}
  %   \label{fig:3dlfm_rabbit}
  % }
  \includegraphics[]{fig1}

   \caption{\centering
   We showcase our spatio-temporal model by lifting a fast-moving, in-the-wild cheetah from noisy 2D pose detections. Both methods were trained on synthetic animal data that did not include a cheetah. Our approach is capable of predicting the fast motion of the cheetah throughout a video sequence. \note{This will go on the first page when I can figure out how to make it work.}
   }
   \label{fig:main}
\end{figure*}

==> legacy/1_intro_mosam_edit.tex <==


Reconstructing 3D structures from 2D landmarks has long been a cornerstone challenge in computer vision. Traditional approaches typically rely on multi-camera setups to address ambiguities. However, recent advances have empowered learning-based methods to lift 3D object structures from sparse 2D keypoints captured by a single camera. These human-centric lifting models, like MotionBERT~\cite{zhuMotionBERTUnifiedPerspective2023a}, have shown remarkable capabilities, primarily due to the availability of vast 3D human pose data. Yet, their reliance on human-specific data and extensive training sets restricts their applicability to non-human objects, particularly animals, where data is scarce.


This limitation has spurred the development of object-agnostic lifting models. Notably, 3D-LFM~\cite{dabhi3DLFMLiftingFoundation2024} pioneered state-of-the-art performance by leveraging diverse object categories and employing transformers with permutation equivariance inductive biases to manage category imbalances and within-category variations. However, a shortfall of 3D-LFM is its inability to utilize temporal information, leading to less accurate reconstructions in dynamic sequences.

Our work tackles these challenges by introducing the first object-agnostic 3D lifting framework that is both data-efficient and temporally aware. Our approach uses the power of transformers with a strategic inductive bias that focuses on temporally proximate frames, enabling it to capture motion dynamics effectively. This approach improves the accuracy of 3D reconstructions across various object categories, even in scenarios with limited data and unseen objects. Additionally, we address the lack of publicly available datasets for diverse animal skeletons and motion sequences by creating a new synthetic dataset. This dataset includes 4D labels for 13 animal categories, encompassing 698 animation sequences with temporal consistency, designed to foster further research in class-agnostic lifting.

The contributions of this paper are: \begin{itemize}
    \item We introduce a class-agnostic 3D lifting model with embedded temporal inductive bias, that shows better performance in scenarios involving noise, occlusions, and unseen objects.
    \item We provide a new synthetic dataset containing 4D skeletons for various animals with animated behavior sequences, prioritizing temporal consistency through a non-linear refinement process.
    \item Finally, we empirically validate the proposed approach on our synthetic dataset, achieving results that outperform competing methods.
\end{itemize}


==> legacy/2_related_works_old.tex <==
\section{Related works}
\label{sec:related_works}

\subsection{3D pose estimation}
There are two primary avenues for obtaining the 3D pose of an object from a single monocular camera. The first is to directly predict the 3D pose from RGB images \cite{brau3DHumanPose2016,park3DHumanPose2016,moonCameraDistanceawareTopdown2019,pavlakosOrdinalDepthSupervision2018}. A drawback of these approaches is poor generalisation to distribution shifts such as lighting and background changes. Alternatively, a two-stage approach leverages the strength of two separate, specialised models \cite{hossainExploitingTemporalInformation2018a,changPoseLifterAbsolute3D2020,liuAttentionMechanismExploits2020,chenAnatomyaware3DHuman2021}. A pose detector extracts the 2D pose of the object and a separated model is used to lift the 2D keypoints into 3D. The two-stage approach is the focus of our paper.

\subsection{Object-specific lifting}
Traditional non-rigid structure-from-motion (NRSfM) algorithms serve well for modelling simple objects like human hands \cite{chenJointwise2D3D2023,ge3DHandShape2019}. A set of 2D keypoints of an object is given, and 3D supervision for the specific object is provided. Recent deep-learning methodologies have shown to be better suited for modelling the complexities of various object rigs \cite{novotnyC3DPOCanonical3D2019a,jiUnsupervised3DPose2023a,wangPAULProcrusteanAutoencoder2021a,kongDeepNonRigidStructure2019a}. However, they are limited by requiring the 2D keypoints to have semantic correspondence across all instances of the object. That is, the index of a specific landmark will always have the same semantic meaning, ie. the elbow of a person. 

This limitation is still present in modern deep-learning models like MotionBERT \cite{zhuMotionBERTUnifiedPerspective2023a} and others \cite{changPoseLifterAbsolute3D2020,chenAnatomyaware3DHuman2021} that are focused solely on human 3D lifting. The specialised nature of these models and their reliance on large datasets make it impractical to apply them to objects with relatively scarce data, like animals. However, 3D lifting models for animals suffer from the same drawback by being specialised for a single category of animal, with the addition of poor generalisation due to scarce data \cite{karashchukAniposeToolkitRobust2021,mathisMarkerlessTrackingUserdefined2018,gosztolaiLiftPose3DDeepLearningbased2020}.

\subsection{Object-agnostic lifting}
A new paradigm of object-agnostic lifting has been recently pioneered by 3D-LFM \cite{dabhi3DLFMLiftingFoundation2024}. It is able to handle a wide variety of object categories at once, leveraging the combination of general information to improve performance for under-represented or totally unseen objects. However, unlike the object-specific models, 3D-LFM does not incorporate temporal information into their approach. Our framework is built upon the best of both worlds.

\subsection{Animal datasets}
In order to benchmark animal-agnostic lifting over video, we require a diverse set of animal categories with accurately labelled 3D skeletons. While recent animal datasets suffice in this regard, they are restricted to single images \cite{xuAnimal3DComprehensiveDataset2024,yaoOpenMonkeyChallengeDatasetBenchmark2023}. Furthermore, there is little species and motion variation among the few publicly available datasets with 3D poses of real animals over video \cite{liPosesEquineResearch2024,chengMarmoPoseDeepLearningBased2024}. Methods to collect data for a broad set of animals has shown to be either impractical, expensive, or produce noisy results.

We instead take inspiration from the tracking community by turning to synthetic data \cite{doerschTAPVidBenchmarkTracking2023a,karaevDynamicStereoConsistentDynamic2023a,zhengPointOdysseyLargeScaleSynthetic2023a}. Available synthetic datasets are restricted to a single animal, like pig \cite{anThreedimensionalSurfaceMotion2023} or ant \cite{plumReplicAntPipelineGenerating2023}, that contain only simplistic motion sequences. The DeformableThings4D \cite{li4DCompleteNonRigidMotion2021} dataset provides complex and diverse motion sequences animated by artists. However, the dataset was created for dense mesh recovery and does not contain the 3D skeletons of animals. We leverage these models and animations to create a new dataset targeting the class-agnostic lifting task.

==> legacy/intro_old1.tex <==
\section{Introduction}
\label{sec:intro}

Reconstructing the 3D structure of a deforming object is an ill-posed problem~\cite{non-rigid-Sfm}. Capturing multiple simultaneous views of an object can help mitigate deformations and thus better constrain the problem~\cite{XXX}. However, this approach necessitates complex and specialized sensor setups in a controlled environment~\cite{XXX}, making it a costly and impractical solution for in-the-wild non-rigid objects, such as humans and animals.

Recently, learning-based methods have emerged as a promising strategy by recasting the reconstruction and modelling of 3D deformable objects as a 2D-3D lifting problem~\cite{XXX}, aiming to recover sparse 3D structure from 2D landmarks. Due to the abundance of 3D human poses provided by the Human3.6M and AMASS datasets, coupled with the lightweight nature of 2D keypoints, this approach has become the dominant method in specialized domain like \note{3D human pose estimation}~\cite{XXX}. \SF{talk about motionbert.}

\SF{Need to improve the transition here}. Notably, 3D-LFM~\cite{XXX} is particularly appealing as it achieves class-agnostic lifting by leveraging the inherent permutation equivariance of transformers. This property enables the model to efficiently lift a wide range of object categories without requiring class-specific training or fine-tuning, while maintaining high fidelity in 3D keypoint estimations. Despite its significant progress on several benchmarks, 3D-LFM does not leverage an important insight: object deformations usually occur in time in practice. We argue that temporal smoothness is crucial for disambiguating rapid motions and occluded viewpoints. 

In this paper we propose \note{XXX}, a method that leverages both joint-to-joint temporal correlation across frames and spatial correlation between joints. This spatio-temporal smoothness offers a significant advantage over 3D-LFM, which only consider the spatial correlation between joints. By enforcing temporal smoothness coupled with a random masking training regime~\cite{XXX}, our approach not only improves the fidelity in 3D keypoint lifting, but also demonstrates enhanced robustness to noisy and/or missing points. More crucially, XXX scales more efficiently in terms of parameters compared to spatial model likes 3D-LFM while maintaining the capability to handle out-of-distribution (OOD) scenarios. 
\note{Additionally, we contribute a new synthetic dataset featuring K species, M animation sequences, and N total frames...refined by non-linear optimization...} Code and data will be released.

The contributions of this paper are:-



==> tables/ood_table_2.tex <==
\begin{table}
  \centering
  {\small{
  \begin{tabular}{@{}l|ccc@{}}
    \toprule
    Method & \text{FA-MPJPE} $\downarrow$ & \text{SA-MPJPE} $\downarrow$ & \text{SA-MPVE} $\downarrow$ \\
    \midrule
    MotionBERT & 132.0 & 142.5 & 6.8 \\
    3D-LFM & 112.0 & 143.4 & 21.9 \\
    Ours & \textbf{75.7} & \textbf{86.4} & \textbf{6.4} \\
    \bottomrule
  \end{tabular}
  }}
  \caption{%\centering
  \textbf{OOD generalization on unseen data.} We perform a $13$-fold evaluation to assess each method's ability to handle unseen animal categories. Our approach demonstrates superior proficiency in handling OOD 2D-3D lifting.  }
  %Out-of-distribution generalisation to unseen animal categories. We evaluate each animal as unseen and report the average.}
  \label{tab:ood_animal}
\end{table}
